On The Open Prompt Challenge In Conditional Audio Generation

Text-to-audio generation (TTA) produces audio from a text description, learning from pairs of audio samples and hand-annotated text. However, commercializing audio generation is challenging as user-input prompts are often under-specified when compared to text descriptions used to train TTA models. In this work, we treat TTA models as a ``blackbox'' and address the user prompt challenge with two key insights: (1) User prompts are generally under-specified, leading to a large alignment gap between user prompts and training prompts. (2) There is a distribution of audio descriptions for which TTA models are better at generating higher quality audio, which we refer to as ``audionese''. To this end, we rewrite prompts with instruction-tuned models and propose utilizing text-audio alignment as feedback signals via margin ranking learning for audio improvements. On both objective and subjective human evaluations, we observed marked improvements in both text-audio alignment and music audio quality.

==> sections/algorithm.tex <==

\begin{algorithm}[htb]
\vspace{0.1cm}
	\caption{Feedback Instruction Learning}
	\label{alg:feedback}
		\begin{algorithmic}[1]
		    \STATE \textbf{Input:}
      Prompt set $\cX=\{x_1,\ldots,x_n\}$, reward function $r(\cdot)$, initial model $G_0 = g(w_0,\cdot)$, acceptance ratio $1/k$, batch size $b$, temperature parameter $\alpha$. %$\lambda$.
			\FOR{Stage $t=1,\dots,T$}
			\STATE {\color{teal} \textbf{\textit{1 . Data collection.}}} Sample a batch $\mathcal{D}_t$ from $\cX$ of size $b$;
            \FOR{$x \in \mathcal{D}_t$}
			\STATE 
            Generate $y \sim p^{\alpha}_{G_{t-1}}$ and compute $r(x,y)$.
             \ENDFOR
    % \STATE {\color{teal} \textbf{\textit{2. Data ranking.}}} Let $\cB$ be the $\lfloor b / k\rfloor$ samples with maximum rewards; 
   % \STATE {\color{teal} \textbf{\textit{3. Model fine-tuning.}}} Fine-tune $w_{t-1}$ on $\cB$ to obtain $G_t = g(w_{t}, \cdot)$.
			\ENDFOR
		\end{algorithmic}
\vspace{0.1cm}
\end{algorithm}


==> sections/figure01.tex <==

\begin{figure}
  \centering
\includegraphics[width=0.8\columnwidth]{emnlp2023-latex/diagrams/audionese_v3.pdf}
\caption{ \small
\textbf{The open prompt challenge:}
Audio descriptive prompts come in different level of expressivity, ranging from expert-annotated musical prompts to user-input prompts, with varying levels of abstraction. The pyramidal shape indicates the ease of annotation where expert-annotation are costly to obtain and are placed at the top as opposed to arbitrary user prompts. 
}
\label{fig:pyramid}
\end{figure}


==> sections/figure04.tex <==

\begin{figure}[h]
  \centering
\includegraphics[width=1\columnwidth]{emnlp2023-latex/diagrams/fig04.pdf}
\caption{ \small 
Plot to indicate the higher CLAP correlation with the proposed technique along information density. }
\label{fig:audionese}
\end{figure}


==> sections/further_plot.tex <==

\begin{figure}[h]
  \centering
\includegraphics[width=1\columnwidth]{emnlp2023-latex/diagrams/further.png}
\caption{ \small . }
\label{fig:further}
\end{figure}


==> sections/inst_template.tex <==

\begin{table*}[h]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{
    \begin{tabular}{p{0.3\linewidth} p{0.2\linewidth}p{0.5\linewidth}}
\toprule
\textbf{User Input} & \textbf{ Instruction} & \textbf{Enhanced Prompt} \\
\midrule
\emph{Write a detailed description describing the music with instruments, tone, pitch, rhythm, atmosphere, style, and all the audio details.}

& \emph{Rewrite the following prompts to be diverse and different}

& \emph{1. Describe the instruments used in the music, including their tone, pitch, and rhythm. 2. Provide details about the overall sound and atmosphere of the music, including the style and genre. 3. Include any special effects or layers that enhance the music, such as layers of guitars or synths.} \\
% \hdashline
\bottomrule
\end{tabular}}
\caption{\small The provided example represents a pair of instruction-input and output generated by instruction-tuned LLMs.}\label{tab:example}
\end{table*}

==> sections/instruction_format.tex <==

\begin{figure}[h]
  \centering
\includegraphics[width=0.6\columnwidth]{emnlp2023-latex/diagrams/instruction_format_v2.pdf}
\caption{ \small  The provided example represents a pair of instruction-input and output that is utilized to train instruction-tuned LLMs.
}
\label{fig:instruction}
\end{figure}


==> sections/table1.tex <==


\begin{table}[hb]
  \small
\centering
\resizebox{0.95\columnwidth}{!}{
\begin{tabular}{lcccccccc}
    \toprule
    & Unseen & Unseen & Unseen & Unseen & Unseen & Unseen & Unseen & Unseen \\ 
    \midrule
% \text{Number of instances} & 40                                                        & 20                                   & 100                                   & 25                                   & 25                                    & 25                                    & 25                                    & 40                                    \\ 
\text{Average number of cells}        & 168.85                                                        & 74.90                                   & 39.46                                   & 27.92                                   & 12.56                                    & 27.6                                   & 34.0                                     & 52.25                                    \\ 
\text{Average number of cells (DL)}          & 3.26                                                        & 2.05                                   & 2.24                                   & 2.44                                   & 3.16                                    & 2.36                                    & 1.68                                     & 2.68                                    \\ 
\text{LS}               & 0.60                                                        & 0.58                                   & 0.59                                   & 0.63                                   & 0.60                                    & 0.61                                    & 0.62                                     & 0.62                                    \\ 
\text{MSTTR}            & 0.56                                                        & 0.60                                   & 0.58                                   & 0.59                                   & 0.60                                    & 0.61                                    & 0.56                                     & 0.61                                    \\ 
 \bottomrule
\end{tabular} }
\caption{ \small caption.}
\label{corpus_stats}
\end{table}
